From Calculation to Adjudication: Examining LLM judges on Mathematical Reasoning Tasks

To reduce the need for human annotations, large language models (LLMs) have been proposed as judges of the quality of other candidate models. The performance of LLM judges is typically evaluated by measuring the correlation with human judgments on generative tasks such as summarization or machine translation. In contrast, we study LLM judges on mathematical reasoning tasks. These tasks require multi-step reasoning, and the correctness of their solutions is verifiable, enabling a more objective evaluation. We perform a detailed performance analysis and find that easy samples are easy to judge, and difficult samples are difficult to judge. Our analysis uncovers a strong correlation between judgment performance and the candidate model task performance, indicating that judges tend to favor higher-quality models even if their answer is incorrect. As a consequence, we test whether we can predict the behavior of LLM judges using simple features such as part-of-speech tags and find that we can correctly predict 70%-75% of judgments. We conclude this study by analyzing practical use cases, showing that LLM judges consistently detect the on-average better model but largely fail if we use them to improve task performance.

==> old/chapters/abstract.tex <==
\begin{abstract}
To reduce the need for human annotations, large language models (LLMs) have been proposed as judges of the quality of other candidate models.
LLM judges are typically evaluated by measuring the correlation with human judgments on generation tasks such as summarization or machine translation.
In contrast, we study LLM judges on mathematical reasoning tasks. These tasks require multi-step reasoning, and the correctness of their solutions is verifiable, enabling a more objective evaluation.
We perform a detailed performance analysis and find that the used judges are mostly unable to improve task performance but are able to pick the better model.
Our analysis uncovers a strong correlation between judgment performance and the candidate model task performance. 
We observe that judges tend to choose the model of higher quality even if its answer is incorrect. 
Further, we show that it is possible to use statistics, such as the task performances of the individual models, to predict judgment performance.
In an ablation, we either swap or mask the candidate answers %(chain of thought, CoT, and answer)
and observe that judges often keep the original judgment, providing evidence that judges incorporate writing style in their judgments.
In summary, we find that regularities in the judgments are quantifiable using statistical measures and provide various angles on exploiting them.\footnote{Code:  \url{git@github.com:AndSt/llm_judges.git}}
\end{abstract}


% To reduce the need for human annotations, large language models (LLMs) have been proposed as judges of the quality of other candidate models.
% LLM judges are typically evaluated by measuring the correlation with human judgments on generation tasks such as summarization or machine translation. In contrast, we study LLM judges on mathematical reasoning tasks. These tasks require multi-step reasoning, and the correctness of their solutions is verifiable, enabling a more objective evaluation.
% We perform a detailed performance analysis and find that the used judges are mostly unable to improve task performance but are able to pick the better model. Our analysis uncovers a strong correlation between judgment performance and the candidate model task performance. We observe that judges tend to choose the model of higher quality even if its answer is incorrect. Further, we show that it is possible to use statistics, such as the task performances of the individual models, to predict judgment performance. In an ablation, we systematically perturb the candidate answers and observe that judges often keep the original answer, providing evidence that judges incorporate writing style in their judgments. In summary, we find that regularities in the judgments are quantifiable using statistical measures, and provide various angles on exploiting them.

% LLM-as-a judge ...

% We want to understand the reliability of reasoning tasks

% Does it get destroyed by CoT?

% does looks on reasoning? -> Writing style -> performance

% experiments -> performance -> writing style


% performance <-> writing style

==> old/chapters/acknowledgements.tex <==
\section{Acknowledgements}

This research was funded by the WWTF through
the project ”Knowledge-infused Deep Learning for
Natural Language Processing” (WWTF Vienna Research Group VRG19-008) and through the project "Transparent and Explainable Models" (WWTF ICT19-041). 
MA is funded by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation) as part of BERD@NFDI - grant number 460037581.
Further, we thank Jan Philip Wahle and Pedro Henrique Luz de Araujo for fruitful discussions and their constructive feedback.

==> old/chapters/conclusion.tex <==
\section{Discussion}

\paragraph{Style and Quality.}

Our experiments suggest a relation between judgment and candidate task performance (cf. Section \ref{sec:subset}) and a relation between judgment and writing style (cf. Sec. \ref{sec:prediction} and \ref{sec:substitution}). We hypothesize these two are interconnected and facets of the same underlying bias.
When models become better, e.g., by being trained on larger amounts of data, their ability to write convincingly increases. 
Conversely, when an LLM demonstrates an increased ability to write convincingly, it likely acquires a more nuanced grasp of what humans perceive as compelling. This enhanced understanding likely also extends to task performance.
%However, on reasoning tasks, judgments should be independent of the writing style.

\paragraph{Generalizability of approach.} 
Our in-depth analysis utilizes Formula \eqref{eq_1} to segment judgment data based on correctness criteria, allowing for targeted investigation of specific subsets. This approach is generalizable and transferable to other NLP tasks, such as summarization. By incorporating discrete signals such as text topics, a similar derivation of the judgment probability is possible.

\section{Conclusion}

We conducted a thorough analysis of LLM judges on mathematical reasoning tasks. We include a detailed judgment performance evaluation of eight models on three datasets. We find that larger models are generally better than smaller models and that judges succeed in detecting the more capable model.
%including results for applied questions such as ``Does the judge prefer the better model?'' and
Our analysis reveals a strong correlation between judgment performance and task performance of the models providing candidate answers which shows that judges tend to choose larger or better models. We hypothesize that LLM judges incorporate writing style into their judgments instead of purely analyzing the reasoning. We provide two experiments to provide evidence for this hypothesis. 

Finally, we want to emphasize the importance of impartiality and fairness in the role of LLM judges, similar to human judges in the real world.
Our research introduces methods to quantify biases in favor of larger or better models, thereby offering a means to measure the reduction of such biases. 


==> old/chapters/experiments_linguistic.tex <==
%\section{Does the substitution of results change judgments?}
\section{Perturbation of Results}
\label{sec:substitution}

\input{tables/linguistically_changed_predictions}

We aim to gain a deeper understanding of the extent to which writing style affects the final judgment. Therefore, we create an experiment perturbing the candidate answers and examine whether this changes the judgment. 

% \paragraph{Setup.} In the \textit{Exchange} experiment, we substitute all occurrences of the final answer in the chain-of-thought reasoning of model $A$ with the final answer of model $B$, and vice versa. 

\paragraph{Setup.} We examine two perturbtations: \textit{Swap} and \textit{Mask}. In the \textit{Swap} experiment, we swap the final answer from model $M_A$ with that of model $M_B$, while keeping their CoT reasoning unchanged. In the \textit{Mask} experiment, we anonymize all numbers in both the CoT reasoning and the final answer by replacing them with ``X''.\footnote{In preliminary runs, we observed that masking caused significant confusion for the judge models. To address this, we adapt the judgment prompt in this setting to include the instruction: ``Only
analyze the reasoning! Therefore we exchanged all numbers with ’X’ so you can focus on the reasoning.''} Table \ref{tab:number_exchange} shows the frequency with which the judge selects the same answer ($=$), a different answer ($\neq$), or fails/refuses to follow the output format and make a decision (Refused). Refer to Appendix \ref{app_sec:substitution_examples} for specific examples.

\paragraph{Results.} 
%Refusals
We observe that the new judgments in more than half the cases agree with the original judgment. In the \textit{Swap} experiment, they even agree on average by 75\% of the cases. We deduce that the judge is largely unaffected by the artificially introduced noise and heavily bases its decision on the writing style.
Interestingly, in a substantial amount of samples (up to $17\%$) the judge refuses to make a judgment. On a positive note, manual inspection revealed that the model often realizes that the original answers were perturbed.
%The model is more likely to refuse when confronted with redacted answers. This is unexpected as this %does not change the logic, but an exchange of answers does. 
% Focus on exchanged, saying weird it doesn't change

==> old/chapters/experiments_performance.tex <==

\section{General Performance}
\label{sec:general_performance}

The experiments have multiple degrees of freedom: judges, candidate models, and datasets. Therefore, we first examine judgments per dataset, and secondly, we investigate judgments per candidate model pair. Afterwards, we provide evaluations for two applied questions.

\subsection{Performance per dataset}

We begin by examining the judgment performance, i.e., how often the judge picks a correct answer across different datasets. Therefore, we average the performance across all model pairs $(M_A, M_B)$.

\paragraph{Setup.} Table \ref{tab:performance_per_dataset} considers three cases where each case focuses on a specific subset of the datasets:
\textit{Case (1)} investigates the observed task performance $P(\Delta_J=T| A, B, D)$ where we evaluate the task performance using the answers chosen by the judges. Note that this includes samples where both candidate models give the same answer.
\textit{Case (2)} asks how often judges choose a correct answer given that the answers differ, i.e., $P(\Delta_J=T| A \neq B, D)$. Note that this may (and often does) include cases where both answers are incorrect.
\textit{Case (3)} gives the probability that the judge chooses the correct answer given that one answer is correct and the other answer is incorrect, formally $P(\Delta_J=T | \{A, B\}=\{T, F\}, D)$. 


\paragraph{Results.}
%Here I say:
% 1) Qwen best, Yi LLama3 70B similar
% 2) (1), (2) bad results, as often many negatives
% 3) Small models around chance -> disregard in further experiments
We observe that large models outperform smaller models. Specifically, we see that Qwen 2 72B is the best judge, followed by Yi 1.5 34B. The performance of Llama 3 70B is, on average, comparable to that of Yi 1.5 34B.
Note that performance in \textit{Case (1)} and Case \textit{(2)} is often quite low, especially for MATH, as there are many cases where the judge can only choose wrong answers. 
Importantly, we observe that smaller models with fewer than 10B parameters are unreliable judges. Especially, in Case (3), where a correct answer is provided, smaller models only achieve an accuracy of around 55\%, barely better than random chance. Therefore, we focus on the four larger models as judges in the subsequent analysis.
%TODO: Say that we will still show experiments for them in appendix.

\input{figures/performance_per_pair}

\subsection{Performance per model combination}

The comparative performance of model pairs offers insights into which model is better for the specific task or which combination of models yields the best results.

\paragraph{Setup.}  Figure \ref{fig:performance_per_pair} illustrates the final performance $P(\Delta_J=T| A, B)$, indicating the probability of a judge choosing a correct answer given two models $A$ and $B$. The results are averaged over datasets and presented as an upper triangular matrix due to symmetry. If both models in a pair are the same, $A=B$, we employ the second response generated with temperature sampling to introduce variation. We report the performance of all models used as judges in the Appendix \ref{app_sec:general_performance} in Table \ref{app_sec:individual_judgements}.
% TODO: Should we add other probabilities in Appendix?

\paragraph{Results.} 
We observe that the best performance is achieved when both the candidate answers and the judge are the highest-performing model, Qwen 2 72B.
An analysis of the first rows (cf. Figure \ref{fig:performance_per_pair}) reveals a notable trend: 
The final performance declines when comparing the output of a strong model against a mediocre model (e.g., Llama3-8B) but then improves again when compared against the weakest model. 
This suggests that judging becomes more challenging when distinguishing between the correct answers of a strong model and the incorrect answers of a mediocre one, compared to discerning the outputs of a bad one.

\subsection{Do judges elicit task improvement?}

\begin{figure}
\centering
\includegraphics[width=0.97\linewidth]{figures/p_j_given_a_b_does_improve.png}
\caption{Amount of model pairs $(M_A, M_B)$ where the answers chosen by the judge achieve a higher task performance than the models individually (green). The blue bar only considers models where the judge is at least as good as the candidate models.}
\label{fig:improve_overall_performance}
\end{figure}

One use case for LLM judges is to improve task performance. A potential application is to train on answers chosen by the judge \cite{yuan2024selfrewardinglanguagemodels}.

\paragraph{Setup.} Therefore, we test how often the performance of the answers chosen by the judge is better than the performance of the individual models. Formally, for all pairs of models $M_A, M_B$ and datasets $D$, how often is the observed performance $P(\Delta_J=T | A, B, D)$ larger than $ \max \{P(A=T | D), P(B=T | D) \}$?
In Figure \ref{fig:improve_overall_performance} the green bar tests all model pairs, and the blue bar only pairs where the judge is at least as good as the candidate models, i.e., 

\noindent
$P(\Delta_J=T|D) \geq \max\{P(A=T|D), P(B=T|D)\}$. The task performances of all models are given in the Appendix 

\ref{app_sec:general_performance} in Table \ref{tab:initial_model_performance_per_dataset}.

\paragraph{Results.} We see that only Qwen 2 72B increases the performance reliably. However, it is easier for the judge to improve performance if it compares answers of less or equally good candidate models.

\begin{figure}
    \centering
    \includegraphics[width=0.97\linewidth]{figures/chooses_better_model.png}
    \caption{Percentage of model pairs $(M_A, M_B)$ where a judge picks a better model $M_A$ (meaning $P(A=T|D)> P(B=T|D)$), by selecting more answers of $M_A$ than from $M_B$.}
    \label{fig:chooses_better_model.png}
\end{figure}

\subsection{Does the judge prefer the better model?}

Another application of LLM judges is whether they can accurately identify which model performs better for a given task. This is crucial if we want to rank LLMs by their capabilities or if a practitioner wants to decide which model to deploy.

\paragraph{Setup.} To assess this, we evaluate the frequency with which a judge selects the superior model. 
For a candidate model pair $M_A, M_B \in \mathbf{M}$, always assume they are ordered, such that $P(A=T| D) > P(B=T | D)$. Then, specifically, we determine the proportion for which the judge chooses $M_A$ more often than $M_B$, or formally, how often is $P(\Delta_J=M_A | A, B, D) > P(\Delta_J=M_B | A, B, D)$ for all candidate pairs and datasets.

\paragraph{Results.}
% Consistently well
The judges consistently perform well in the selection of the better model.
% Larger models better
% Qualitatively, we find reasons why it sometimes does not work:
Notably, we find that Qwen 2 72B can only not rank the pair Mistral 7B v0.1 and v0.3 on the MATH dataset. This issue appears minor, as both models exhibit similarly poor performance on the challenging MATH dataset (with accuracies of $6.13\%$ and $3.10\%$, respectively), meaning most judgments compare two wrong answers. Notably, already the worst judge, Mixtral 8x7B, performs well.
In summary, we see that judges are more capable of aggregate-level rankings than instance-level rankings.

==> old/chapters/experiments_predictions.tex <==
\input{tables/r2_correctness}

\section{Prediction of Judgements}
\label{sec:prediction}

We investigate whether predicting the judgments' outcomes is feasible. Firstly, we aim to predict performance statistics. Secondly, we aim to predict individual judgments.

\subsection{Can we predict judgment performance?}

On the subset where exactly one answer is correct, we found a strong correlation between judgment performance and candidate task performances.
This hints at regularities within the judging process, thus we aim to predict judge performance using model statistics.

\paragraph{Setup.} We fit six different linear regression models using the judgment performances as the target variables $Y$, including all variations of judges, model pairs $M_A, M_B \in \mathbf{M}$, and datasets $D$. Regarding the covariates $\mathbf{X}$ in the model, we distinguish between two setups: In \textit{Case (1)}, we solely use the task performances $P(X|D), X \in \{J, A, B\}$ of judge and candidate models, to predict judgment performance. In \textit{Case (2)}, we utilize statistics available without knowledge of the ground truth. The features for this case are the probability of agreement between the candidate models $P(A=B|D)$ and the probability of model $M_A$ being chosen. Since we are not specifically interested in the individual features' effects, but rather in their ability to explain the variation of judgment performance, we rely on the coefficient of determination, $R^2$, for evaluation \citep[][, see Appendix \ref{a:stats}]{fahrmeir2013regression}.

\paragraph{Results.} The results are shown in Table \ref{tab:exp_r2_overview} (excluding data sets from the probability formulas for simplicity). We observe that the performance-related features of the models can almost perfectly explain the variation in final judgment performance ($R^2 = 97.50\%$), also when conditioning only on the subset of differing answers ($R^2 = 90.20\%$). Logically, $P(A)$ and $P(B)$, i.e., $P(A|D), P(B|D)$ respectively, have significant\footnote{We test statistical significance using an Overall-F-Test for each fitted model. Further details are in Appendix \ref{a:stats}.} explanatory power for judgment performance, as they encompass all correct answers. In \textit{Case (2)}, we still observe a relatively high $R^2$ value, indicating that the features can explain 50\% of the target's variance.

% \input{figures/predict_judging_given_performances}
\input{tables/predict_judgement}

\subsection{Can we predict which individual judgments?}

We hypothesize that judgments are biased towards larger or better models because they incorporate linguistic cues or writing style into their judgments rather than purely relying on reasoning assessment. Therefore, we train a classifier to understand whether we can predict individual judgments.

\paragraph{Setup.} We separate all comparisons made per judge into training, validation, and test splits and train two classifiers. The test accuracy is reported in Table \ref{tab:predict_judgement}.
The first model utilizes TF-IDF vectorization. We create two independent vectorizers for both answers. The resulting features are concatenated. A RandomForest classifier \cite{breimanrandomforests} is then trained on these combined features.
The second model is a RoBERTa model \cite{liu2020roberta} trained on the full prompt presented to the judge. Refer to Appendix \ref{app_sec:individual_judgements} for the training details of both models.

\paragraph{Results.} The random forest model achieves an accuracy of approximately 60\%, demonstrating performance above random chance. This suggests that specific keywords or phrases influence judges.
The RoBERTa model surpassed this, reaching nearly 70\% accuracy. 
Taken together, these results suggest that judge decision-making is a multi-faceted process. While specific linguistic cues appear to hold influence, a substantial portion of the decision-making process seems to be based on other contextual factors or broader reasoning.

==> old/chapters/experiments_subset.tex <==
\input{figures/performance_diff_vs_accuracy}

\section{Analysis of Subsets}
\label{sec:subset}

We investigate properties that occur when we use subsets based on the correctness of models or agreement between models.

%TODO: Better motivation
%Naively, $P(J=T| A,B,S_1) \approx P(J=T| A,B,S_2)$ for two subsets $S_1, S_2 \subset D$ would ensure that we can assume similar performance on new similar data. In this analysis, we test how far this holds true. We base the definition of $S_1, S_2$ on the correctness of $A, B$.

\subsection{Do task performances correlate with judgments?}

We consider the subset of highest practical relevance where one candidate model is correct, and one candidate model is incorrect. 
%In this experiment, we consider the subset of cases with the highest practical relevance where A is correct and B is not, or vice versa.
The goal is to investigate the relationship between candidate model task performance and judgment performance.

\paragraph{Setup.} For all model pairs $M_A, M_B \in \mathbf{M}, M_A \neq M_B$ we analyze subsets where $M_A$ is correct, and $M_B$ is incorrect. Note that we can always order $M_A$ and $M_B$ this way.
Each plot in Figure \ref{fig:performance_diff_vs_accuracy} shows the relationship between judge performance, $P(\Delta_J=T | A=T, B=F)$ (Y-axis) and candidate model performance gap of $M_A$ and $M_B$, i.e., $P(A=T| D) - P(B=T | D)$ (X-axis). Examples of these subsets and their corresponding performances are in Appendix \ref{app_sec:subset} in Table \ref{tab:subset_examples}.

\paragraph{Results.} The analysis reveals a strong correlation (Pearson's $r^2 > 0.69$) between candidate model performance gap and judgment accuracy. If the performance gap is negative, we consider subsets where larger models are incorrect.
Judges favor answers from larger models even when they are incorrect on these subsets. We hypothesize that this bias arises because larger models exhibit a specific writing style, articulating their responses more convincingly, thereby misleading the judges. 
This finding aligns with previous research identifying self-bias \cite{xu2024prideprejudicellmamplifies, panickssery2024llmevaluatorsrecognizefavor, liu2024llmsnarcissisticevaluatorsego}. However, our results indicate that this bias extends more broadly to the inherent quality of the underlying models on reasoning datasets.
However, this is not necessarily a critical issue in practice, as the larger model tends to answer correctly more often (as indicated by the color of the points in Figure \ref{fig:performance_diff_vs_accuracy}.


\subsection{Do judgments relate to own answers?}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/performance_given_judge_answer_in_options}
    \caption{For the comparisons, where the judge gave the same answer as one of the compared models, i.e., $J \in \{A, B\}$, how often does he choose his initial answer, given that it was correct or incorrect?}
    \label{fig:performance_given_judge_answer_in_options}
\end{figure}

Furthermore, we investigate whether there is a relationship between the answer generated by the judge and the answers it must compare. [TODO: motivation]

\paragraph{Setup.} The analysis incorporates all samples where the judge's initial answer is one of the two compared answers, i.e.,  $J \in \{A, B\}$. We restrict the analysis to instances where the two models provide different answers, i.e., $A \neq B$. Figure \ref{fig:performance_given_judge_answer_in_options} illustrates the probabilities that the judge selects their initial answer, denoted as $\Delta_J = J$, across three conditions: (1) the initial answer $J$ is correct, (2) the initial answer $J$ is incorrect, with both $A$ and $B$ being incorrect and (3) the initial answer $J$ is incorrect, but either $A$ or $B$ is correct.

\paragraph{Results.} In case (1), when the judge's initial prediction is correct, there is a high likelihood that the judge selects the answer that it also gave initially. Note that this set also likely represents an easier set of questions where judgment is easier.
In case (2), if the judge's initial prediction is incorrect but there is a correct alternative, judges show a modest tendency to select the correct answer. However, they still choose their incorrect initial answer, approximately 40\%-50\%. We follow that this set is more challenging so the judgement performance is rather low.
In case (3), where both answers are incorrect, judges predominantly choose their own initial answers, with this tendency being stronger in larger models.
Overall, these findings indicate a bias in the judging process, where the initial prediction unduly influences the final decision.

% \subsection{Does judgment quality depend on models' agreement?}

% \input{figures/performance_given_agreement}

% We are interested in whether the level of agreement among models, i.e., how many models give a different answer for a sample, impacts the performance on the respective subset.

% \paragraph{Setup.} We define disagreement buckets $S_j$, where each bucket contains instances for which exactly $1 \leq j \leq 8 $ unique answers were given across all models. Formally, we set

% {\small
% \begin{align*}
%     S_j = \bigcup_{D} \left\{ i \in D \mid |\{M_A(i) \mid M_A \in \mathbf{M}\}| = j \right\}
% \end{align*}
% }

% where $M_A(i)$ is the answer of model $M_A$ for instance $i$. We analyze the results in two contexts: all comparisons, including those where both answers are correct or incorrect (cf. Figure \ref{fig:performance_by_agreement}(a)), and only instances where exactly one answer is correct (cf. Figure \ref{fig:performance_by_agreement}(b)). We average the performances of all judges and all candidate pairs. Find per-judge plots in Appendix \ref{app_sec:subset} in Figure \ref{fig:performance_by_agreement_full}.

% \paragraph{Results.} 
% % Fig a)
% Figure \ref{fig:performance_by_agreement}(a) shows that when all models agree (bucket $S_1$), the performance is nearly 100\%, indicating unanimous agreement usually means correctness. As disagreement increases, performance expectedly decreases.
% Thus, model agreement is a proxy for sample difficulty.
% % Fig b)
% In \ref{fig:performance_by_agreement}(b), where a correct and an incorrect answer exists, performance remains relatively stable across disagreement buckets for datasets with free-form answers, such as GSM8K and MATH. However, for AQUA-RAT, performance degrades as disagreement rises. 
% %[TODO: Takeaaway]

==> old/chapters/interesting_examples.tex <==
Question:
Helen went on a trip through Germany. She booked a hotel for 3 nights and rode the bus 7 times during that trip. One night at the hotel was a cost of \$80, and every bus trip was 10\% of the price of one night at the hotel. How much did Helen pay for the hotel and bus travels during that trip?

Answer A:
The cost of one night at the hotel is \$80.
So, the total cost for the hotel is 3 * \$80 = <<3*80=240>>240.
The cost of one bus trip is \$80 * 10/100 = <<80*10/100=8>>8.
So, the total cost for bus trips is 7 * \$8 = <<7*8=56>>56.
Therefore, Helen paid \$240 + \$56 = <<240+56=306>>306 for the hotel and bus travels during her trip to Germany.
#### 306
--------------
Answer B: 
The cost of one bus trip was 0.1 * 80 = \$<<0.1*80=8>>8.
So Helen paid 3 * 80 = \$<<3*80=240>>240 for the hotel.
And she paid 7 * 8 = \$<<7*8=56>>56 for the bus trips.
So Helen paid a total of 240 + 56 = \$<<240+56=296>>296 for the hotel and bus travels.
#### 296
--------------

B is correct, models choose A. Answer is more "direct", as things appear more in order as in original question

==> old/chapters/introduction.tex <==
\section{Introduction}

The automatic evaluation of machine learning models promises to reduce the need for human annotations. Specifically, the LLM-as-a-judge paradigm \cite{zheng2023judging} has gained traction, aiming to assess or compare the quality of generated texts automatically. This approach is beneficial for automated data labeling \cite{tan2024largelanguagemodelsdata}, self-improvement of LLMs \cite{wu2024metarewardinglanguagemodelsselfimproving}, and ranking LLMs with respect to specific tasks \cite{zheng2023judging}.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/figure_1.pdf}
    \caption{In our problem setup two LLMs ($M_A$ and $M_B$), 
    provide candidate answers for a math problem, and a judge LLM \textit{has} to decide which one is correct. All three use chain-of-thought (CoT) reasoning \cite{wei2022chain}.}
    \label{fig:figure1}
\end{figure}


Much like judges in the real world, who are expected to be exact, fair, and unbiased, e.g., as defined in Bangalore Principles of judicial conduct \cite{bangalore_principles}, LLMs, when employed as judges, should be ethical and logical.
%While the approach holds great potential, it is039 essential to investigate the behavior of judges to un-040 derstand their properties, and biases [CITE]
% Characterize current approaches that tackle the same problem and highlight their shortcomings (as related to your approach)
Already the philosopher Aristotle argued that the virtuous actor exhibits the joint excellence of reason and character \cite{sep-aristotle-ethics}.
Previous works investigate properties and biases of LLM judges on generation tasks such as translation or summarization \cite{kim2024biggen, liu2024llmsnarcissisticevaluatorsego}. These are typically evaluated using correlation with human annotators and are thus inherently subjective.

% Describe the main novelty of your approach
In this work, we investigate LLM judges on mathematical reasoning datasets (see Figure \ref{fig:figure1}). These need complex multi-step reasoning, and the solution is verifiable, which allows us to investigate the relationship between judge and candidate models in a principled manner.
%We derive insights into judgment performance on reasoning tasks and whether a judge actually reasons to select the better answer or whether linguistic cues or writing styles impact the decision.
% Describe your methodology
We base our analysis on four large (more than 30B parameters) LLMs and four small (less than 10B) LLMs on three mathematical reasoning datasets. %We first experiment with all combinations of judges and compare models and find that only large models are competent judges. The subsequent analysis is one of them.

% Performance
Our experiments contain a detailed performance examination, confirming that larger models are generally better judges \cite{zheng2023judging}. We find that only the best-tested model, Qwen 2 72B, consistently improves task performance if we evaluate the judged samples, but all tested judges likely pick the better model for a given task.

%Subsets
We investigate subsets with one correct and one incorrect candidate answer. We uncover a correlation between judgment performance and task performance of the candidate models, showing that judges tend to select incorrect answers from better models. Thus, we hypothesize that judges have access and rely on the superior \textit{writing styles} of larger models instead of solely analyzing the reasoning.
When we divide the datasets into buckets of model agreement, we observe that agreement is a proxy for sample difficulty. % and that judgment performance remains relatively stable on the subset of samples with one correct and one incorrect candidate answer.

% Prediction
Motivated by these regularities, we analyze whether it is possible to predict judgment performance and find that task performances of judge and candidate LLMs explain most of the variance.
We hypothesize that judges incorporate writing style into their judgments. Thus, we predict individual judgments using statistical and transformer-based models and achieve above-chance performance, supporting our hypothesis.

% Substitution
Lastly, we test how judgments are affected by perturbing numeric values in responses by 1) swapping results and 2) masking numeric values. Our findings reveal that judges largely retain original judgments, providing further evidence that judges, in large part, base their decisions on writing style.
%Highlight the main insight
In summary, our contributions are as follows:
% [TODO: this is shit]
% [STORY: performance -> interesting subsets (we see and hypothesize that Y) -> based on this we make predictions to verify Y -> further we adapt initial experiment to verify Y]

\begin{enumerate}
\item We conduct an in-depth performance analysis of LLM judges for mathematical reasoning tasks.
\item Our analysis reveals a correlation between the judgment and candidate task performance, providing a novel statistical angle on the analysis of LLM judges.
\item We show that statistics such as task performance or agreement of candidate models are indicative of judgment performance.
% [high level. statistics <-> writing style bridge possible???]
\item After systematically perturbing the candidate answers, we observe that judges often keep their original judgments, providing evidence that judgments are also based on writing style.
\end{enumerate}

==> old/chapters/limitations.tex <==
\section*{Limitations}

Our analysis is primarily focused on mathematical reasoning datasets, which allows us to explore judgments through the lens of correctness within specific subsets. While this approach provides valuable insights, it limits the generalizability of our findings to other tasks or domains. 
Based on the fact that the investigated datasets are complex, in the sense that they need multi-step reasoning to be solved, and based on the fact that there is no thorough investigation of LLM judges on mathematical reasoning datasets yet, we think this work is a valuable contribution. 

In our experiments, we focus on testing a single, specific prompt. It is common knowledge that LLMs are highly sensitive to variations in prompt phrasing, which can substantially influence their performance. Nevertheless, it is impossible for us to meet the computational demands necessary to run our experiments with multiple prompts.
%Future studies could incorporate a variety of prompts to better understand the robustness and consistency of LLM judgments under different conditions. This would provide a more comprehensive evaluation of their reasoning assessment.

In this study, we intentionally concentrate on open-weight models, motivated by our strong belief in the principles of open science. Open-weight models offer transparency and reproducibility, which are critical for advancing scientific understanding. However, we note that it is also interesting to study closed models to understand potential differences.
Still, we are committed to research on open-weight models because we believe it benefits the community more.
% However, it is worth noting that an analysis of closed models might yield interesting insights. 
% Closed models are thought to be trained on larger and more sophisticated preference-tuning datasets, which may enhance their capabilities in terms of judgment accuracy and bias mitigation. It is an interesting research direction whether our results extend to those models.


==> old/chapters/related_work.tex <==
\section{Related Work}

\subsection{LLM as Judges}

Using \emph{LLMs as judges} to evaluate text generated by LLMs, including their own outputs, has recently attracted significant interest because it reduces the need for human annotation \cite{zheng2023judging}. Commonly, large \emph{frontier models} are used as judges. Applications include the automatic assessment of language model capabilities and, e.g., determining which model performs better on a given task \cite{zheng2023judging} and reinforcement learning from AI feedback by automatically generating data for preference optimization \cite{bai2022constitutional, wu2024metarewardinglanguagemodelsselfimproving}.

Various methods exist to make judgments \cite{zheng2023judging, liusie-etal-2024-llm}. One approach is pairwise selection \cite{wang2024pandalm}, where two answers are presented, and the model is asked to select the better one. Another approach is pointwise grading \cite{li2024generative}, where the model is asked to assign a grade based on a predefined scale, and the answer with a better grade is chosen. 
%Additionally, it is possible to compare the likelihoods assigned by a judge to different solutions. [TODO: Find or remove, not really called LLM-as-judge] 
Judgment prompts may involve reference solutions or not.
Another body of research explicitly trains models to act as judges \cite{kim2024prometheus, wang2024pandalm} or closely related, as reward models \cite{wang2024helpsteer2, li2024generative}. 
%However, our work focuses on open-weight models without specific evaluation fine-tuning.

The effectiveness of LLMs as judges is typically assessed by measuring the correlation or overlap with human judgments \cite{zheng2023judging, kim2024biggen}. In contrast, we focus on difficult tasks with a concrete final answer. 
Finally, we want to stress that several works caution for the use of LLM judges as experts \cite{bavaresco2024llmsinsteadhumanjudges, koo2023benchmarkingcognitivebiaseslarge, raina2024llmasajudge}. 
In a similar vein, we aim to understand regularities and their shortcomings.

\subsection{Biases in LLM-as-a-judge}

Human-annotated data inherently reflects the annotators' biases and opinions. These biases can be detrimental or (intentionally) beneficial, depending on the goals of the annotation process \cite{plank-2022-problem}. Similarly, several studies have explored the biases present in LLM judges:

One linguistic bias is ordering bias \cite{zheng2023judging, koo2023benchmarkingcognitivebiaseslarge}, where a judge gives a different answer depending on the order in which answers are presented. \citet{panickssery2024llmevaluatorsrecognizefavor} note that it is possible to interpret position bias as a sign that the model is unsure. 
There are multiple works \cite{xu2024prideprejudicellmamplifies, panickssery2024llmevaluatorsrecognizefavor, liu2024llmsnarcissisticevaluatorsego} that find evidence for self-bias or self-preference.
\citet{koo2023benchmarkingcognitivebiaseslarge} provide a benchmark for analyzing cognitive biases.
\citet{west2024the} and \citet{oh-etal-2024-generative} explore the ``Generative AI Paradox'' where generating solutions is easier for the LLM than analyzing them, unlike humans who typically find analysis easier than generation.

% For next paragraph; motivate ours
In this work, we aim to establish a better understanding of underlying regularities that relate judgments to statistics such as model performance.

% \subsection{Predicting generalization performance}

% There is also research on predicting the performance of machine learning (ML) models based on statistical properties. 

% Cite Koller et al. \cite{yao2023predicting}

% This work differentiates itself by exploring the intersection of these two areas.
% Maybe something from statistics?

% Maybe something about understanding CoT
% M

==> old/chapters/setup.tex <==
\section{General Setup }
\label{sec:setup}

In the following, we describe the problem setting, including the used notation, and the general experimental setting including used models and datasets.

\subsection{Problem Description}

In this work, we consider two models, denoted by $M_A, M_B \in \mathbf{M}$, providing candidate solutions for a sample of a dataset $D$ and a judge model $M_J \in \mathbf{M}$, which is tasked to select, to ``judge'' whether both answers are correct or incorrect or if an individual answer is correct. Thus, the task is a four-way classification.

% prefers the solutions of the models $M_A$ or $ M_B$. The solutions are represented by the random variables $A$ and $B$. We consider the events that solutions are true $(A=T)$, false $(A=F)$, or that their solution is the same $(A=B)$.
% We denote the judgment of the judge $M_J$ by the random variable $\Delta_J$, which can either be correct $(\Delta_J=T)$, incorrect $(\Delta_J=F)$ or choose a specific model $M_A$ $(\Delta_J=M_A)$.

% Given that the final answer is either correct or incorrect, we can break the probability of the judge making a correct judgment $P(\Delta_J=T | A, B, D)$ given a sample of a dataset $D$ and the answers of two models $M_A, M_B$ down into four cases

% {\scriptsize 
% \begin{align}
% % \fontsize{4pt}{4pt}\selectfont
% &P(\Delta_J | A, B, D) \label{eq_1}\nonumber  \\
% &= \sum_{(X, Y), X, Y \in \{T, F\}} P( \Delta_J=T | A=X, B=Y, D) P(A=X, B=Y|D) \nonumber \\
% % &= P(\Delta_J | A=T, B=F, D) P(A=T, B=F|D)\nonumber \\
% % &+ P(\Delta_J=T | A=T, B=F, D) P(A=T, B=F|D)\nonumber \\
% % &+ P(\Delta_J=T | A=F, B=T, D) P(A=F, B=T|D)\nonumber
% \end{align}
% }

% Note that in cases where both answers are correct or incorrect imply that the judgment is also either correct or incorrect respectively, i.e., $P(\Delta_J=T | A=T, B=T)=1$ and $P(\Delta_J=T | A=F, B=F)=0$. 
%We will analyze the judgment performance and the judgement performance on interesting subsets, such as, e.g., $P(\Delta_J=T | A=T, B=F, D)$.

% Therefore, we focus on analyzing $P(Delta_J=T | A, B, D)$ as a whole, and we focus on the interesting cases where one model is correct, and the other model is interesting

% \textbf{Discussion. } 
% [TODO Discussion about setup here??]
% - it is a realistic setup (Citations), solving applied ...
% - It simplifies analysis
% - Other variants ... but would complicated ...
% {\small 
% \begin{align*}
% % \fontsize{4pt}{4pt}\selectfont
% &P(J=T | D, I_A + I_B=1)  \\
% &+ P(J=T | A=T, B=F, D) &P(A=T, B=F|D) \\
% &+ P(J=T | A=F, B=T, D) &P(A=F, B=T|D)
% \end{align*}
% }
% where $I_A=1$ if $A=True$, $0$ otherwise.


\subsection{Datasets}

The experiments encompass three mathematical reasoning datasets where models highly benefit from multi-step CoT reasoning. For all datasets, we use accuracy as the performance metric.\\
\textbf{AQUA-RAT} \cite{ling-etal-2017-program} is a dataset to test the quantitative reasoning ability of LLMs. Unlike the other two datasets, the questions are multiple-choice. 
\textbf{GSM8K} \cite{cobbe2021gsm8k} consists of grade school math word problems. The answers are free-form numbers. 
\textbf{MATH} \cite{hendrycksmath2021} contains challenging competition mathematics problems. Find more details in Appendix \ref{app_sec:datasets}

\subsection{Models}

We evaluate the performance of openly available LLMs, including four large models \textit{Qwen 2 72B} \cite{qwen2}, \textit{Llama 3 70B} \cite{llama3modelcard}, \textit{Yi 1.5 34B} \cite{ai2024yi}, \textit{Mixtral 8x7B} \cite{jiang2024mixtralexperts} and four small models, namely \textit{Llama 3 8B} \cite{llama3modelcard}, \textit{Gemma 1.1 7B} \cite{gemmateam2024gemmaopenmodelsbased}, \textit{Mistral 7B v0.3} \cite{jiang2023mistral7b}, and \textit{Mistral 7B v0.1} \cite{jiang2023mistral7b}. We use the chat- or instruction-tuned model variants and test each model as a candidate answer generator and as a judge. More information is in Appendix \ref{app_subsec:models}.

\subsection{Inference}

This section describes the candidate answer generation and the judgment generation. Find more information on prompts and hardware details in Appendix \ref{app_sec:experimental_setup}.

\paragraph{Candidate answer generation.} To judge two candidate answers (including of the same model), we sample two initial CoT solutions for each model using 4-shot prompting. We set the temperature to $0.9$ to get two different solutions.

\input{tables/performance_per_dataset}

\paragraph{Judgements.} For each model pair and for each dataset, we generate one judgment. We choose the first candidate generation for each model and generate judgments for all $36$ unique model combinations.\footnote{We consider all pairs from the eight LLMs, including self-pairing, yielding $\binom{8+2-1}{2}=36$ combinations.} 
If both models are the same, we also take the second generated candidate answer.
We accommodate positional bias \cite{zheng2023judging, koo2023benchmarkingcognitivebiaseslarge} by evaluating the two candidate answers in both possible orders for each question and then taking the average correctness of the judgments to assess performance.
%Using zero-shot prompting, we ask the model to first reason about both answers using CoT and then choose if the first answer (Option $A$) or the second answer (Option $B$) is correct. 
% The judge \textit{has} to choose if the first or second answer is correct. The prompt is zero-shot and applies CoT, the temperature is set to 0 for deterministic generation results.


==> old/figures/performance_diff_vs_accuracy.tex <==
\begin{figure}[t]  % Adjust placement as needed (h = here, t = top, b = bottom, p = separate page)
\centering
\begin{subfigure}{0.231\textwidth}  % 0.3 for three images, adjust for different numbers
\centering
\includegraphics[width=\textwidth]{figures/performance_diff_vs_accuracy/Qwen_Qwen2-72B-Instruct.png}
\caption{Qwen2 72B}%: Pearson correlation coefficient $0.76$.}
\end{subfigure}
%\hfill  % Add space between images
\begin{subfigure}{0.22\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/performance_diff_vs_accuracy/meta-llama_Meta-Llama-3-70B-Instruct.png}
\caption{LLama2 70B}%: Pearson correlation coefficient $0.73$.}
\end{subfigure}
\begin{subfigure}{0.231\textwidth}  % 0.3 for three images, adjust for different numbers
\centering
\includegraphics[width=\textwidth]{figures/performance_diff_vs_accuracy/01-ai_Yi-1.5-34B-Chat-16K.png}
\caption{Yi 1.5 43B}
\end{subfigure}
\begin{subfigure}{0.22\textwidth}  % 0.3 for three images, adjust for different numbers
\centering
\includegraphics[width=\textwidth]{figures/performance_diff_vs_accuracy/mistralai_Mixtral-8x7B-Instruct-v0.1.png}
\caption{Mixtral 8x7B}
\end{subfigure}
\caption{Judges' accuracy vs. performance gap between two candidate models $M_A$ and $M_B$. Each point represents a subset where $M_A$ is correct and $M_B$ is incorrect. The color reflects the size of these subsets.}
\label{fig:performance_diff_vs_accuracy}  % Label for referencing the figure
\end{figure}

==> old/figures/performance_given_agreement.tex <==
\begin{figure}%[h]
\centering
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/performance_given_agreement_all.png}
    \label{fig:performance_by_agreement_a}
    \caption{Performance on all comparisons.}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/performance_given_agreement_corr_incorr.png}
    \label{fig:performance_by_agreement_b}
    \caption{Performance on comparisons with one correct and one incorrect answer.}
\end{subfigure}
\caption{Judge performance by agreement bucket. E.g., bucket $S_3$ (X-axis) means that all eight models gave together three different answers. Note that AQUA-RAT is multiple-choice with maximally six answers.}
\label{fig:performance_by_agreement}
\end{figure}


==> old/figures/performance_per_pair.tex <==
\begin{figure}%[h]
\centering
\begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/performance_per_pair/Qwen_Qwen2-72B-Instruct.png}
    \caption{Qwen 2 70B}
\end{subfigure}
\begin{subfigure}{0.226\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/performance_per_pair/meta-llama_Meta-Llama-3-70B-Instruct.png}
    \caption{LLama3 70B}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/performance_per_pair/01-ai_Yi-1.5-34B-Chat-16K.png}
    \caption{Yi 1.5 34B}
\end{subfigure}
\begin{subfigure}{0.226\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/performance_per_pair/mistralai_Mixtral-8x7B-Instruct-v0.1.png}
    \caption{Mixtral 8x7B}
\end{subfigure}
\caption{Observed performance $P(\Delta_J=T|A, B, D)$ of four judge LLMs (a-d) in evaluating various model pairs, averaged across all datasets.}
\label{fig:performance_per_pair}
\end{figure}


==> old/figures/predict_judging_given_performances.tex <==
\begin{figure}[t]  % Adjust placement as needed (h = here, t = top, b = bottom, p = separate page)
\centering
\begin{subfigure}{0.22\textwidth}  % 0.3 for three images, adjust for different numbers
\centering
\includegraphics[width=\textwidth]{figures/predict_performance_p_j_given_a_b/model_Qwen2-72B.png}
\caption{Qwen2 72B}%: Pearson correlation coefficient $0.76$.}
\end{subfigure}
%\hfill  % Add space between images
\begin{subfigure}{0.22\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/predict_performance_p_j_given_a_b/model_Llama-3-70B.png}
\caption{LLama2 70B}%: Pearson correlation coefficient $0.73$.}
\end{subfigure}
\begin{subfigure}{0.22\textwidth}  % 0.3 for three images, adjust for different numbers
\centering
\includegraphics[width=\textwidth]{figures/predict_performance_p_j_given_a_b/model_Yi-1.5-34B.png}
\caption{Yi}
\end{subfigure}
\begin{subfigure}{0.22\textwidth}  % 0.3 for three images, adjust for different numbers
\centering
\includegraphics[width=\textwidth]{figures/predict_performance_p_j_given_a_b/model_Mixtral-8x7B.png}
\caption{Mixtral}
\end{subfigure}
\caption{We train on the performances of three judges and predict the held-out one. The graphs show prediction errors.}
\label{fig:predict_given_individual_performances}  % Label for referencing the figure
\end{figure}

==> old/tables/initial_model_performances.tex <==
\begin{table}
    \centering
\resizebox{0.48\textwidth}{!}{
    \begin{tabular}{lrrr}
\toprule
 & AQUA-RAT & GSM8K & MATH \\
\midrule
Qwen 2 72B & 76.38 & 92.04 & 51.19 \\
Llama 3 70B & 73.62 & 91.05 & 34.37 \\
Yi 1.5 34B & 64.96 & 78.47 & 27.04 \\
Mixtral 8x7B & 47.24 & 61.18 & 13.79 \\
Llama 3 8B & 51.18 & 73.01 & 15.04 \\
Gemma 1.1 7B & 42.91 & 50.72 & 12.60 \\
Mistral 7B v0.3 & 38.19 & 42.76 & 6.13 \\
Mistral 7B v0.1 & 21.65 & 26.08 & 3.10 \\
\bottomrule
\end{tabular}
}
\caption{Task performance of all models using the prompt in Figure \ref{fig:initial_prompt}.}
\label{tab:initial_model_performance_per_dataset}
\end{table}

==> old/tables/linguistically_changed_predictions.tex <==
\begin{table}
    \centering
\resizebox{0.47\textwidth}{!}{
    \begin{tabular}{l|rrr|rrr}
\toprule
& \multicolumn{3}{c|}{Swapped} & \multicolumn{3}{c}{Masked} \\ 
 & = & $\neq$ & Refused  & = & $\neq$ & Refused \\
\midrule
Qwen2-72B & 75.75 & 12.20 & 12.05 & 56.40 & 26.06 & 17.53 \\
Llama-3-70B & 78.81 & 13.72 & 7.47 & 63.44 & 29.22 & 7.33 \\
Yi-1.5-34B & 74.80 & 14.47 & 10.73 & 44.89 & 37.31 & 17.80 \\
Mixtral-8x7B & 71.19 & 20.69 & 8.12 & 60.34 & 29.26 & 10.40 \\
\bottomrule
\end{tabular}
    }
    \caption{Analysis of judgments where results in candidate answers were either swapped or numbers masked. We report how many judgments stay the same $(=)$, different $(\neq)$, or where judges refused to follow the output format (Refused). }
    \label{tab:number_exchange}
\end{table}

==> old/tables/performance_per_dataset.tex <==
\begin{table*}[t]
    \centering
\resizebox{.97\textwidth}{!}{
    \begin{tabular}{ll|cccc|cccc}
\toprule
 &  & Qwen 2 72B & Llama 3 70B& Yi 1.5 34B & Mixtral 8x7B & Llama 3 8B & Gemma 1.1 7B & Mistral 7B v0.3 & Mistral 7B v0.1 \\
\midrule
\multirow{3}{*}{(1) $P(\Delta_J=T |A, B, D)$} & AQUA\_RAT & \textbf{66.05} & 55.98 & \underline{62.2} & 57.08 & 51.59 & 53.52 & 54.96 & 51.41 \\
 & GSM8K & \textbf{77.06} & 72.41 & \underline{72.64} & 68.81 & 65.88 & 65.47 & 68.57 & 63.28 \\
 & MATH & \textbf{29.66} & 24.64 & \underline{26.69} & 23.60 & 22.35 & 21.66 & 22.68 & 19.91 \\
\cline{1-10}
\multirow{3}{*}{(2) $P(\Delta_J=T |A \neq B, D)$} & AQUA\_RAT & \textbf{53.79} & 45.04 & \underline{49.73} & 44.47 & 36.56 & 40.48 & 38.26 & 36.43 \\
& GSM8K & \textbf{63.16} & \underline{59.33} & 56.01 & 46.68 & 41.29 & 38.71 & 42.59 & 39.72 \\
 & MATH & \textbf{25.04} & 22.14 & \underline{22.22} & 18.29 & 17.04 & 16.00 & 16.88 & 15.22 \\
\cline{1-10}
\multirow{3}{*}{(3) $P(\Delta_J=T | \{A, B\}=\{T, F\}, D)$} & AQUA\_RAT & \textbf{73.13} & 64.63 & \underline{68.66} & 63.26 & 52.74 & 58.04 & 54.54 & 52.45 \\
 & GSM8K & \textbf{85.65} & \underline{81.32} & 76.84 & 64.97 & 57.87 & 54.16 & 59.58 & 55.48 \\
 & MATH & \textbf{80.48} & \underline{73.01} & 71.37 & 61.03 & 58.04 & 54.70 & 56.27 & 50.91 \\
\bottomrule
\end{tabular}
}
\caption{Performance of judge LLMs in three cases: (1) accuracy on all samples, (2) accuracy where models $M_A$ and $M_B$ disagree, and (3) accuracy where only one model is correct. Results are averaged over all pairs $(M_A, M_B)$, with the highest accuracy in bold and the second highest underlined.}
\label{tab:performance_per_dataset}
\end{table*}

% \caption{Performance of judges ($\Delta_J=T)$ of all samples (1), samples where answers of $A$ and $B$ differ (2) and samples where answers differ and one answer is correct (3), averaged over all combinations of models $A, B$. Best performance is in bold. }

==> old/tables/predict_judgement.tex <==
\begin{table}[t]
\centering
\resizebox{.47\textwidth}{!}{
\begin{tabular}{l|rrrr}
\toprule
$\downarrow$ Model  \textbackslash Judge $\rightarrow$ & Qwen 2 72B & Llama 3 70B & Yi 1.5 34B & Mixtral 8x7B \\
\midrule
(1) TF-IDF + RF & 60.78 & 61.37 & 60.77 & 58.69 \\
(2) RoBERTa & 68.14 & 66.49 & 67.03 & 63.91 \\
\bottomrule
\end{tabular}
}
\caption{Accuracy of predicting LLM judges' decisions using Random Forest (RF) and RoBERTa classifiers.}
\label{tab:predict_judgement}
\end{table}

==> old/tables/r2_correctness.tex <==
\begin{table}
    \centering
    \resizebox{.47\textwidth}{!}{
\begin{tabular}{llrrr}
        & & \multicolumn{3}{c}{$P(\Delta_J=T \;|\; \mathcolorbox{pink}{\textcolor{pink}{\cdots\cdots}})$}\\
    \toprule
        \multicolumn{2}{l}{↓ Features \textbackslash\; Condition →} & $\mathcolorbox{pink}{A,B}$ & $\mathcolorbox{pink}{A \neq B}$ & $\mathcolorbox{pink}{\{T, F\} = \{A, B\}}$ \\
    \toprule
        (1) & $P(J), P(A), P(B)$ & 97.50 & 90.20 & 59.20 \\
    \midrule
        \multirow{2}{*}{(2)} & $P(A=B)$, & \multirow{2}{*}{76.00} & \multirow{2}{*}{54.90} & \multirow{2}{*}{49.90} \\
        &$P(\Delta_J=A | A \neq B)$ &&&\\
    \bottomrule
\end{tabular}
    }
\caption{Coeffictions of Determination ($R^2$, higher is better) for linear regression using the different feature sets as covariates (rows) and different target variables defined by the condition (columns). All values are significant ($p < 0.001$) as per an Overall-F-Test.}
\label{tab:exp_r2_overview}
\end{table}

% \begin{table}
%     \centering
%     \resizebox{.47\textwidth}{!}{
% \begin{tabular}{llrrr}
%     %     & & \multicolumn{3}{c}{$P(\Delta_J=T \;|\; \mathcolorbox{pink}{\textcolor{pink}{\cdots\cdots}})$}\\
%     % \toprule
%         \multicolumn{2}{l}{↓ Features \textbackslash\; Target →} & All & Unequal & 1-correct \\
%     \toprule
%          & $P(J), P(A), P(B)$ & 97.50 & 90.20 & 59.20 \\
%     % \midrule
%     %     \multirow{2}{*}{(2)} & $P(A=B)$, & \multirow{2}{*}{76.00} & \multirow{2}{*}{54.90} & \multirow{2}{*}{49.90} \\
%     %     &$P(\Delta_J=A | A \neq B)$ &&&\\
%     \bottomrule
% \end{tabular}
%     }
% \caption{Coeffictions of Determination ($R^2$, higher is better) for linear regression using the different feature sets as covariates (rows) and different target variables defined by the condition (columns). All values are significant ($p < 0.001$) as per an Overall-F-Test.}
% \label{tab:exp_r2_overview}
% \end{table}

==> old/tables/unfollowed_format.tex <==
\begin{table}
    \centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lrrrr}
\toprule
judge & T, T & T, F & F, T & F, F \\
\midrule
Qwen 2 72B & 21.57 & 3.09 & 7.30 & 15.99 \\
Llama 3 70B & 48.50 & 3.00 & 4.55 & 10.89 \\
Yi 1.5 34B & 28.45 & 4.54 & 7.74 & 15.22 \\
Mixtral 8x7B & 17.97 & 6.82 & 8.18 & 9.78 \\
Llama 3 8B & 16.53 & 4.19 & 4.50 & 3.63 \\
Gemma 1.1 7B & 6.81 & 1.72 & 1.97 & 1.45 \\
Mistral 7B v0.3 & 3.12 & 5.68 & 6.37 & 6.40 \\
Mistral 7B v0.1 & 36.12 & 20.39 & 21.32 & 25.55 \\
\bottomrule
\end{tabular}
}
    \caption{Caption}
    \label{fig:unfollowed_format}
\end{table}
